MulTi-Wise Sampling: Trading Uniform T-Wise Feature Interaction Coverage for Smaller Samples

Ensuring the functional safety of highly configurable systems often requires testing representative subsets of all possible configurations to reduce testing effort and save resources. The ratio of covered t-wise feature interactions (i.e., T-Wise Feature Interaction Coverage) is a common criterion for determining whether a subset of configurations is representative and capable of finding faults. Existing t-wise sampling algorithms uniformly cover t-wise feature interactions for all features, resulting in lengthy execution times and large sample sizes, particularly when large t-wise feature interactions are considered (i.e., high values of t). In this paper, we introduce a novel approach to t-wise feature interaction sampling, questioning the necessity of uniform coverage across all t-wise feature interactions, called \emph{\mulTiWise{}}. Our approach prioritizes between subsets of critical and non-critical features, considering higher t-values for subsets of critical features when generating a t-wise feature interaction sample. We evaluate our approach using subject systems from real-world applications, including \busybox{}, \soletta{}, \fiasco{}, and \uclibc{}. Our results show that sacrificing uniform t-wise feature interaction coverage between all features reduces the time needed to generate a sample and the resulting sample size. Hence, \mulTiWise{} Sampling offers an alternative to existing approaches if knowledge about feature criticality is available.

==> 002_sections/acks.tex <==
%This work was supported by funding from the topic Engineering Secure Systems of the Helmholtz Association (HGF) and by KASTEL Security Research Labs (46.23.03).
%This publication is also partially based on the research project SofDCar (19S21002), which is funded by the German Federal Ministry for Economic Affairs and Climate Action.
%The authors would like to thank the Ministry of Science, Research and Arts of the Federal State of Baden-Württemberg for the financial support of the projects within the Innovations Campus Future Mobility (ICM).
%We thank Niklas Mund for developing first concepts and prototype implementation during his master thesis. 
%We also thank Tim Witschel and Elias Kuiter for providing the framework implementations to analyze KConfig-based variability models.

%This work was supported by funding from the topic \grantKASTEL~(\grantNumKASTEL).
%This publication is also partially based on the research project \grantSofDCar~under the grant number \grantNumSofDCar.
We thank the \grantICM~for the financial support of the projects within the Innovations Campus Future Mobility (ICM).
This work is partially funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) – SFB 1608 – 501798263.
%We thank Piotr Malkowski for helping with the implementation of our concepts.


==> 002_sections/concept_backup.tex <==
\subsection{Problemstatement}
T-wise feature interaction coverage is a prominent metric to rate the effectiveness of samples for testing product lines\cite{VAT+:SPLC18}. 
%Many software failures are caused by the interaction of selected and deselected features rather than the presence or absence of a single feature. 
Testing a set of configurations that achieve full (100\%) t-wise feature interaction coverage for high values of \twiseText (i.e., $\twise = 3$, $\twise = 4$, $\twise = 5$, etc.) promises a high chance of discovering a fault in a product line. 
Modern sampling algorithms such as \yasa{} can calculate samples that achieve t-wise feature interaction coverage for various values of \twiseText (e.g., $\twise = 1$, $\twise = 2$, $\twise = 3$, $\twise = 4$, etc.)~\cite{KTS+:VaMoS20}. 
However, generating samples that achieve full t-wise feature interaction coverage for higher values of \twiseText (i.e., $\twise > 2$) becomes more time-consuming and results in more configurations with an increasing t-value because exponentially more feature interactions must be considered when generating a sample.
For instance, using the \yasa sampling algorithm to generate a pair-wise ($\twise = 2$) sample for our running example takes only a few milliseconds, and the resulting sample contains seven configurations.
In contrast, calculating a sample that achieves three-wise feature interaction coverage ($\twise = 3$) takes three seconds, and the resulting sample contains 18 configurations. 
%, while generating a four-wise ($\twise = 3$) sample takes about 3 seconds. 
%The time it takes to generate a sample for larger feature models increases exponentially, as known from the combinatorial explosion problem~\cite{HNA+:EMSE19}.  
%Besides the challenge of generating a sample that achieves high t-wise feature interaction coverage, testing all configurations contained by the resulting sample poses another challenge. 
%With an increasing t-value, generated samples that achieve full t-wise feature interaction coverage tend to contain drastically more configurations compared to samples that achieve full t-wise feature interaction coverage for smaller values of \twiseText because achieving full t-wise feature interaction coverage for higher values of \twiseText requires that more combinations of features are covered in the resulting sample.
%For instance, a sample for our running example generated with the \yasa sampling algorithm that achieves pair-wise feature interaction coverage contains seven configurations. 
%In contrast, a sample that achieves three-wise feature interaction coverage contains 18 configurations.
While calculating a sample in three seconds and testing 18 configurations seems manageable, for larger systems, the number of configurations increases exponentially with the number of optional features in the feature model~\cite{HNA+:EMSE19}. 
In industry branches where testing each configuration requires lots of monetary resources (i.e., safety-critical cyber-physical systems), testing an enormous number of configurations is not feasible. 
Therefore, the challenges of increasing the time to generate samples and the increase in the number of configurations for testing limit the application of samples, achieving full (100\%) t-wise feature interaction coverage for higher values of t (i.e., $t > 2$).
%Instead, selecting configurations for testing often relies on expert knowledge, which leads to an unstructured testing process.

\subsection{Solution Idea}
In practice, certain groups of features exist that are potentially more valuable to cover with higher t-wise feature interactions. 
For instance, covering the feature interactions between a group of features that share highly interconnected implementation artifacts with higher values of \twiseText is probably more valuable than doing so for features that do not share any implementation artifacts.
Other examples of more valuable feature groups include safety-critical features of a system and recently changed features. 
%Building those feature groups depends on expert knowledge of the system. 
%The concept behind Adaptive Sampling is to utilize expert knowledge for a structured test process utilizing t-wise feature interaction coverage samples. 
The concept behind \mulTiWise{} is to generate samples that cover the features of relevant feature groups with high t-wise feature interaction coverage. 
In contrast, features in non-relevant groups are covered with lower t-wise feature interaction coverage.
%We aim to achieve high t-wise feature interaction coverage within groups of features identified as valuable. 
%The feature interaction coverage for other feature groups is intentionally low. 
%
In our running example, the features implementation of \texttt{Carbody}, \texttt{Manual}, and \texttt{Automatic} strongly interact with each other. 
Therefore, they belong to a critical feature group for which the testing requirement defines pair-wise coverage.
The features \texttt{Car}, \texttt{Radio}, and \texttt{Gearbox} are important to certain customers. 
They belong to a feature group requiring one-wise feature interaction coverage. 
For the remaining features, no special t-wise feature interaction coverage is required.
%
%For instance, we can define that all recently changed features belong to a single feature group and that a resulting sample achieves three-wise (t=3) feature interaction coverage for this group of features. 
%We can also define that the resulting sample will achieve at least one-wise (t=1) coverage for features not included in the group of recently changed features.
%We expect to reduce the size of samples by covering only valuable feature interactions with higher values of t.  
%Trading off the idea of generating a sample that achieves 100\% t-wise feature interaction coverage with high values of t (T > 2) for all features against doing so only for a selected group of features introduces the risk of missing faults. 
%However, adaptive sampling allows an informed trade-off between taking a higher risk of missing faults and having a higher testing effort (e.g., testing more configurations). 

%We utilize feature attributes~\todoTP{CITE feature attributes} to express expert knowledge for features.
%Further, we define a dynamic concept for grouping features based on feature attributes and a concept to build a t-wise feature interaction coverage sample based on those feature groups.  

\subsection{Feature Grouping}
%Adaptive sampling relies on expert knowledge to prioritize features from a feature model and categorize them into t-wise feature interaction groups. 
\mulTiWise{} uses t-wise feature interaction groups as a basic concept to generate samples.
We define a t-wise feature interaction group $\tGroupLHS = \tGroupRHS | \tGroupLHS \subseteq \featureSpaceLHS$ as a set of features from the feature model $\model$. 
We define the set of all t-wise feature interaction groups as $\tGroupSetLHS = \tGroupSetRHS$. 
$\tGroupDefault$ represents a default t-wise feature interaction group that contains all features from the feature set $\featureSpaceLHS$ that are not contained in any other t-wise feature interaction group.
A feature $\feature \in \featureSpaceLHS$ can simultaneously be part of multiple t-wise feature interaction groups.
The union, $\bigcup \tGroupSetLHS = \featureSpaceLHS$ of all t-wise feature interaction groups, is equal to the set of all features defined by the feature model.
We assign a t-wise feature interaction coverage value $\twiseText$ to each $\tGroupLHS$.
Multiple t-wise feature interaction groups may have the same t-wise feature interaction value. 

%% table that shows t-wise feature interaction groups for the running example
\input{../004_tables/tgroupExample.tex}
%%

\autoref{tab:groupingTable} shows an example of t-wise feature interaction groups for our running example. 
We define three t-wise feature interaction groups, of which one is the default group.
Each group gets assigned a t-wise feature interaction value ($\twise$), shown in column two of \autoref{tab:groupingTable}. 
Column three shows which features from the feature model are assigned to each group.  
For instance, in \autoref{tab:groupingTable}, we see that $\tGroupLHS_1$ contains the features \texttt{Car}, \texttt{Radio}, \texttt{Gearbox} and that this group has a t-value of $\twise = 1$ assigned. 
The features \texttt{Carbody}, \texttt{Manual}, and \texttt{Automatic} are in $\tGroupLHS_2$ with a t-value of $\twise = 2$. 
The default t-wise interaction group $\tGroupDefault$ contains the features \texttt{USB}, \texttt{CD}, \texttt{Ports}, \texttt{Navigation}, \texttt{Bluetooth}, which are not assigned to any other t-wise feature interaction group in our example. 
We assign a t-value of one ($\twise = 0$) to the default t-wise feature interaction group, meaning that considering interactions between those features for the resulting sample is optional. 
%\begin{itemize}
%    \item We use feature attributes~\todoTP{CITE feature attributes} to assign a feature to t-wise feature interaction groups. 
%    \item A feature $f$ can be annotated with multiple feature attributes simultaneously. 
%    \item Therefore, we define the set of feature attributes a feature can have as $\mathcal{A}_f$. 
%    \item We define a feature attribute $fa_{key} \in \mathcal{A}_f$ as tuple $fa = (key, value)$ consisting of a $key$ and a $value$ property.
%    \item The key-property ($key$) is a string value that uniquely identifies a feature attribute $fa_{key}$ in the set of feature attribute $\mathcal{A}_f$. 
%    \item The value-property ($value$) can be of any type (e.g., Boolean, String, Integer, or a Set of values). 
    %\item It represents the expert knowledge encoded in the feature attribute $fa_{key}$. 
%    \item Using this tuple representation, feature attributes can be used to express any meta-knowledge an expert may have about a feature.
%    \item For instance, a domain expert can annotate that a feature was recently changed by using a feature attribute $fa_{changed} = (string, Boolean)$, where a Boolean value of \texttt{true} represents a recent change and a \texttt{false} value represents no change. 
%    \item Other applications of feature attributes include annotating a feature with a cost factor (i.e., $fa_{cost} = (string, double)$), a risk value (i.e., $fa_{risk} = (string, double)$), or with a categorization based on implementation artefacts (i.e., $fa_{atrefact} = (string, string)$). 
%    \item For adaptive sampling, directly annotating features with t-values is the most convenient use of feature attributes. 
%    \item \autoref{tab:featureAttributes} shows an example of annotating the features of our running example with feature attributes that represent t-values. 
%    \item Each feature from our running example gets a certain t-value assigned. 
    %\item Based on those t-values, all features can be categorized into the four t-wise feature interaction groups $Tgroup_{t=1} = {Feature1}$, $Tgroup_{t=2} = {Feature2}$, $Tgroup_{t=3}  = {Feature3}$, and $Tgroup_{t=4}  = {Feature4}$. 
%\end{itemize}

%\begin{table}
%    \centering
%    \caption{Feature annotation for the car running example using feature attributes to represent t-values.}
%    \begin{tabular}{*3c} \toprule
%        Feature ID & Feature name  & $fa_{t-value}$ \\ \hline
%        1 & Feature 1 & 1 \\
%        2 & Feature 2 & 2 \\ 
%        3 & Feature 3 & 3 \\ 
%        4 & Feature 4 & 4 \\ \bottomrule
%    \end{tabular}    
%    \label{tab:featureAttributes}
%\end{table}

%\begin{itemize}
%    \item Directly annotating features with t-values makes assigning features to t-wise feature interaction groups straightforward.
%    \item For our running example, we can derive the four t-wise feature interaction groups $Tgroup_{t=1} = t=1, 1, {Feature1}$, $Tgroup_{t=2} = t=2, 2, {Feature2}$, $Tgroup_{t=3}  = t=3, 3, {Feature3}$, and $Tgroup_{t=4}  = t=4, 4, {Feature4}$. 
%    \item However, assigning features to t-wise feature interaction groups based on annotated t-values is often not feasible in practice because it is inflexible and requires high effort in practice. 
%    \item For instance, each feature can only be assigned to one t-wise feature interaction group, and changing the assignment requires changing the feature attribute in the feature model.
%    \item Therefore, we define $g : F \rightarrow TGROUP$ as a context-depend grouping function that uses logical conditions $\phi(f)$ using the feature attributes ($fa$) of $f$ to assign $f$ to t-wise feature interaction groups.  
%    \item \autoref{eq:grouping} shows the formal definition of our grouping function $g$. 
%    \item We define a logical condition $\phi_{tg}(f) \in \Phi$ for each t-wise feature interaction group in $TG$.
%    \item The set of all grouping conditions is defined $\Phi$.
%    \item If the feature attributes $fa$ of a feature $f$ fulfill the condition defined by $\phi_{tg}$, the feature is assigned to the respective t-wise feature interaction group $tg$. 
%    \item If the feature attributes $fa$ of a feature $f$ fulfill multiple conditions $\{\phi_{1}, \phi_{2}, \dots, \phi_{n}\} \subseteq \Phi$ the feature $f$ is assigned to all fulfilling t-wise feature interaction groups. 
%    \item If the feature attributes $fa$ of a feature $f$ do not fulfill any condition $\phi_{tg} \in Phi$, the feature $f$ is assigned to the default t-wise feature interaction group $tg_{0}$.
%\end{itemize}

%\begin{equation} \label{eq:grouping}
%    g(x) = \begin{cases} 
%        \{tg_1\} & 
%        \begin{split}
%            & \text{if } \phi(f) \text{ is true for group } tg_1 \in TG  
%        \end{split}
%        \\[5pt]
%        \{tg_2\} & 
%        \begin{split}
%            & \text{if } \phi(f) \text{ is true for group } tg_2 \in TG  
%        \end{split}
%        \\
%        \vdots
%        \\
%        \{tg_k\} & 
%        \begin{split}
%            & \text{if } \phi(f) \text{ is true for group } tg_k \in TG  
%        \end{split}
%        \\[5pt]
%        \{tg_0\} &
%        \begin{split}
%            & \text{otherwise, if } \phi(f) \\ 
%            & \text{ is false for all groups in } TG
%        \end{split}
%    \end{cases}
%\end{equation}

%\begin{lstlisting}[caption={Example configruation for assigning features to feature groups.},captionpos=t, label=lst:groupConf]
%    ### Definition of feature groups ###
%    defGroup{
%    tg1, 1;
%    tg2, 2;
%    tg3, 3;
%    tg4, 4;
%    }
%    ### Definition of conditions ###
%    defCon{
%    If (t-value == 1) then t1; 
%    If (t-value == 2) then t2;
%    If (t-value == 3) then t3;
%    If (t-value == 4) then t4;
%    }
%\end{lstlisting}

%\begin{itemize}
%    \item We realize the grouping function as a Java command line application that takes a configuration file and an attributed feature model as input parameters. 
%    \item In the configuration file, users of our application define the feature groups and the conditions to assign features to the feature groups. 
%    \item The file environment \texttt{defGroup{\dots}} defines t-wise feature interaction groups. 
%    \item Inside the curly brackets, the t-wise feature interaction groups are defined following the syntax \texttt{group id, group t-value}. 
%    \item A semicolon marks the end of defining a t-wise feature interaction group.   
%    \item \autoref{lst:groupConf} shows a grouping configuration for our running example, which defines the four t-wise feature interaction groups tg1, tg2, tg3, tg4 with their respective t-values 1,2,3,4.
%    \item The conditions $\phi(f)$ are defined in between the curly brackets of the \texttt{defcon{\dots}} environment. 
%    \item The syntax of a condition follows an \texttt{If(statement) then groupId;} structure, where \texttt{groupId} must be defined in the \texttt{defGroup{\dots}} environment, and the semicolon marks the end of a condition definition. 
%    \item The \texttt{statement} of the \texttt{If()} block can be an arbitrarily complex concatenation of logical expressions over feature attributes using logical AND () and OR () as connectors between them.
%    \item Each expression expresses a logical relation between a feature attribute $fa$ by listing its key property and a value of a certain type.
%    \item For the logical relations we allow value equality check \texttt{==}, as well as smaller (\texttt{<}, \texttt{<=}) and larger (\texttt{>}, \texttt{>=}) as checks. 
%    \item In \autoref{lst:groupConf}, we define four conditions to assign features of our running example to the respective t-wise feature interaction group. 
%    \item Each condition queries a feature for its \texttt{t-value} property and checks if the value of this property is equal to one, two, three, or four. 
%    \item Depending on the conditions' result, the feature is assigned to the t-wise feature interaction group tg1, tg2, tg3, or tg4. 
%    \item 
%\end{itemize}

\subsection{Generating a Sample}
\label{subsec:sampling}

\autoref{alg:adaptiveSampling} shows a pseudocode algorithm to visualize the generation process for a sample using adaptive sampling. 
Adaptive sampling uses a feature model ($\model$), as well as a set of t-wise feature interaction groups ($\tGroupSetLHS$) as input to generate a sample ($\samp$). 
The resulting sample achieves t-wise feature interaction coverage for all given t-wise feature interaction groups for the respective t-value of each group.
In the case of our running example, the resulting sample will achieve one-wise feature interaction coverage for the features in $\tGroupLHS_1$ and pair-wise feature interaction coverage for the features of $\tGroupLHS_2$. 
Since we defined no specific t-wise coverage (i.e., a t-value of zero) for $\tGroupDefault$, our algorithm does not guarantee a certain t-wise coverage for the included features.

%% pseudocode algorithm for adaptive sampling
\input{../004_pseudoCodes/adaptive-algo.tex}
%%
Our algorithm iterates over the set of t-wise feature interaction groups provided as input (see line 1).
As shown in line 2 of the pseudocode, our algorithm extracts the t-value of the respective t-wise interaction group. 
After that, the algorithm generates an intermediate sample $\samp'$ that achieves the respective t-wise feature interaction coverage for the features in the current feature interaction group (see line 3).
The final step of our algorithm (see line 4) merges the intermediate sample $\samp'$ with the global result sample $\samp$ by adding all configurations from $\samp'$ to $\samp$ that do not already exist in $\samp$.

We use the covering strategy of the existing YASA sampling algorithm~\cite{KTS+:VaMoS20} to generate the intermediate sample $\samp'$ of \autoref{alg:adaptiveSampling}. 
YASA is an efficient t-wise sampling technique that provides various options when calculating samples that achieve t-wise feature interaction coverage~\cite{KTS+:VaMoS20}
For instance, the YASA algorithm can generate a sample that achieves t-wise feature interaction coverage for only a subset of features from the feature model. 
We use exactly this functionality of YASA to calculate intermediate samples for each t-wise feature interaction group. 

%% pseudocode algorithm for a basic sampling algorithm
%%
\input{../004_pseudoCodes/basic-t-wise.tex}
%%
%%
We present the basic covering strategy of the YASA sampling algorithm in \autoref{alg:basicSampling}. 
The algorithm takes the feature model $\model$, a t-wise coverage value $\twise$, and a set of features $\tGroupLHS$ as input and generates a sample $\samp$ as output. 
The algorithm starts by generating a set of all valid feature interaction tuples $\intersetLHS{\twise}{\model}{\tGroupLHS}$ of size $\twise$ for the feature set $\tGroupLHS$ (see line 1). 
%% table showing the interaction sets for the TGroups from the TGroup example table
%%
\input{../004_tables/interactionsets.tex}
%%
%%
\autoref{tab:interactionTable} shows the valid interaction tuples for the example t-wise feature interaction groups presented in \autoref{tab:groupingTable}. 
We present the features of our running example in their literal notation to keep a concise representation. 
Generating feature interaction tuples for $\tGroupLHS_1$ results in four feature tuples of size. 
The features \texttt{Car} (i.e., 1) and \texttt{Gearbox} (i.e., 3) are mandatory features in our running example. 
Therefore, the feature interaction tuples $\neg 1$ and $\neg 3$ are excluded from \autoref{tab:interactionTable}. 
Two one-wise feature interaction tuples (e.g., $2$ and $\neg 2$) are valid For feature \texttt{Radio} because it is an optional feature in our running example.
Algorithm \autoref{alg:basicSampling} generates six valid pair-wise feature interaction tuples for $\tGroupLHS_2$, resulting from the specified t-value $\twise = 2$ and the constraints of the feature model. 
The set of generated feature interaction tuples for $\tGroupDefault$ is empty because our example specifies a t-value of $\twise = 0$ for this group, which means that no specific t-wise feature interactions between the features in this group must be considered when generating a sample.

Then, it iterates over all interaction tuples (see line 2) and checks for each interaction tuple $\interactionLHS_{n}$ whether this tuple is already covered in any configuration of the sample $\samp$. 
The algorithm proceeds with the next interaction tuple $\interactionLHS_{n+1}$ if a configuration contains the interaction tuple $\interactionLHS_{n}$.
Otherwise, it iterates over the set of existing configurations in $\samp$ and tries adding $\interactionLHS_{n}$ to the currently selected configuration $\conf'$ so that the result is still valid with regard to the feature model (see lines 3 to 5). 
If the resulting configuration $\conf'$ is still valid, $\conf'$ replaces the original configuration $\conf$ in the sample, and the algorithm continues with the next interaction tuple (see lines 6 to 9). 
Otherwise, the interaction tuple $\interactionLHS$ is added to the sample $\samp$ as a new partial configuration (see line 13). 
Finally, the algorithm completes each partial configuration in $\samp$ by selecting or deselecting all undecided feature options so that the partial configurations in $\samp$ become complete and valid configurations with regard to the feature model $\model$. 
%% table showing the results from applying adaptive sampling to the example feature interaction groups
%%
\input{../004_tables/exampleSample.tex}
%%
%%
In \autoref{tab:exampleSample}, we show the stepwise process of generating a sample with adaptive sampling. 
As we show in \autoref{alg:adaptiveSampling}, adaptive sampling is an iterative process that generates an intermediate sample for t-wise feature interaction groups and uses them further in the sampling process.
In the case of our running example, adaptive sampling starts with calculating an intermediate sample for $\tGroupLHS_1$. 
Covering all feature tuples for $\tGroupLHS_1$ (see the first row of \autoref{tab:interactionTable}) requires two partial configurations (visualized with green color in \autoref{tab:exampleSample}). 
For our running example, we complete partial configurations by deselecting as many features as possible to have a deterministic and comprehensible approach to completing partial configurations.
In practice, more sophisticated completion strategies can reduce the total number of configurations for large systems.
After the sample for $\tGroupLHS_1$ is generated, we generate an intermediate sample that covers the feature interactions identified for $\tGroupLHS_2$ (see the second row of \autoref{tab:exampleSample}).
We use the intermediate sample generated for $\tGroupLHS_1$ as input. 
The previously generated configurations $\conf_1$ and $\conf_2$ already cover three of the six feature interaction tuples for $\tGroupLHS_2$ (visualized with green color). 
Our procedure generates a third configuration to cover the remaining feature interaction tuples of $\tGroupLHS_2$ (visualized with green color) to finalize the intermediate sample for this iteration. 
The default t-wise feature interaction group $\tGroupDefault$ of our running example does not introduce new t-wise feature interaction tuple that needs to be covered by adaptive sampling. 
Therefore, our procedure generates no more configurations and returns a final sample containing the configuration $\conf_1$, $\conf_2$, and $\conf_3$ visualized in the last row of \autoref{tab:exampleSample}. 

==> 002_sections/metric.tex <==
In this section, we define continuous t-wise coverage as an extension of t-wise coverage and argue, how our definition satisfies the requirements of \autoref{sec:probstate}.

\subsection{Defining Commit and Sample Histories}
We capture a systems' evolution by its commit history $\commitHistoryLHS$.
A commit $\commitLHS$ represents all changes done by a developer to create a new system version.
%Those changes can either affect the problem space, the solution space, or both at the same time.
We define the commit history as list of commits $\commitHistoryLHS = \commitHistoryRHS$, which describes all changes to the system throughout its history. 
Naturally, we define the length of the commit history $\commHistSizeLHS = \commHistSizeRHS$ as the number of commits contained in the commit history. 
The first element in the list (i.e., $\commitLHS_{0}$) is the earliest commit of the system, while the last element in the list (i.e., $\commitLHS_{\commHistSizeLHS}$) represents the most recent commit of the system. 
In our running example (see \autoref{sec:probstate}), we have a commit history containing three commits, starting with \texttt{commit 0} at index $\commitLHS_{0}$ and ending with \texttt{commit 2} at index $\commitLHS_{2}$.

In sample-based testing, tests are executed on a number of selected system configurations (i.e., a sample $\samp$). 
Over the systems' evolution, a history of tested samples is built, which we define as the sample history $\sampleHistLHS = \sampleHistRHS$ of the system. 
In case of our running example, $\sampleHistLHS$ contains three samples, i.e., $\sampleHistLHS = \listOpen \{c1, c2, c3\}, \{c4, c5, c6\}, \{c7, c1, c2\} \listClose$.
A sample is tested for each commit of the system. 
We define the size of $\sampleHistLHS$ to be equal to the the length of $\commitHistoryLHS$.
Further, we got a one-to-one mapping between the elements of $\commitHistoryLHS$ and $\sampleHistLHS$.
Using this mapping, we can query a sample $\samp_{h} \in \sampleHistLHS$ from the sample history by a commit $\commitLHS_{h} \in \commitHistoryLHS$ from the commit history.

\subsection{Defining Continuous T-Wise Coverage}
\label{subsec:metricDef}
As defined in \autoref{eq:osCoverage}, t-wise interaction coverage is measured as the ratio between feature tuples contained in the configurations of a sample and all possible feature tuples of the respective commit.
Our new metric, \textit{continuous t-wise coverage}, extends this definition of by considering a sequence of samples (i.e., a sample window $\sampleWindowLHS$) instead of a single sample.
The size of this sequence (i.e., the size of the sample window) can be adapted to any number of available samples in the sample history $\sampleHistLHS$.
\autoref{eq:ctwc} shows the resulting formula to calculate continuous t-wise coverage.

\begin{equation}\label{eq:ctwc}
	\begin{split}
		\contCovLHS
		& = \contCovRHS \\
		& = \conCovLHSalt
	\end{split}
\end{equation}

Recall that the function $I$ only considers valid and unique interactions. 
%Therefore, we can reuse the same feature model $\mathcal{M}$ for all samples in the history.
Hence, per definition all invalid feature tuples caused by problem space changes are excluded from the calculation of continuous t-wise coverage so that continuous t-wise coverage satisfies the robustness requirement (Req.4).
As the function $I$ is defined using sets, computing the union of samples from the sample window yields itself a set of unique configurations, maintaining a correct number of covered interactions, even if they are covered by multiple sample configurations in different samples (i.e., continuous t-wise coverage satisfies Req.3)
Furthermore, as the union of samples in the history constitutes a sample itself, it holds that the continuous coverage of a sample window $\sampleWindowLHS$ of size one equals the classic coverage, which satisfies the first requirement Req.1.

\subsection{Customization Options}
\label{subsec:params}
An application of continuous t-wise coverage is to support the efficient usage of testing resources by determining how many configurations must be tested per commit for achieving t-wise feature interaction coverage in a fixed number of commits. 
We define the parameters window size $\windowSizeLHS$ and sample size $\testSampleSize$ to make continuous t-wise coverage adaptable for differing testing requirements.

We introduce the commit window $\commitWindowLHS$ to adjust the number of considered commits when calculating continuous t-wise coverage. 
The commit window $\commitWindowLHS$ is a sub-sequence of the commit history.
We define the size of the commit window $\windowSizeLHS = \abs{\commitWindowLHS}$ as the number of commits the commit window contains. 
All commits in the commit window are ordered as a list of elements $\commitWindowLHS = \commitWindowRHS$, starting with the most recent commit of the commit history $\commitLHS_{\commHistSizeLHS}$ and ending with the n-th most recent commit counting backwards.
Similar we define the sample window $\sampleWindowLHS = \sampleWindowRHS$.
In our running example, the commit window $\commitWindowLHS$ is equal to its commit history $\commitHistoryLHS$. 
However, we can imagine another example where only two commits (i.e., $\windowSizeLHS = 2$) in the  running example are considered to calculate continuous t-wise coverage. 
In this case, the commit window contains the third and the second commit $\commitWindowLHS = \listOpen \text{commit2}, \text{commit1} \listClose$ and the respective sample window contains the configurations $\sampleWindowLHS = \listOpen  \{c1,c2,c7\}, \{c4,c5,c6\}\listClose$.

%\subsection{Tailoring the Sample Size}
We define the number of configurations of a sample $\samp$, by $\testSampleSize$.
With this sample size parameter, we can choose how many configurations of a sample are tested in each commit. 
Consequently, $m = 3$ for our running example.
%
The commit window size $\windowSizeLHS$ and the sample size $\testSampleSize$, provide the freedom to experiment with various strategies to achieve t-wise feature interaction coverage over time.
Hence, our metric can be applied flexibly to various testing scenarios, which satisfies the adaptability requirement Req.2.

%\rework{
%\subsection{Considering Solution Space Changes}
%As described earlier, continuous t-wise coverage partially satisfies the robustness requirement (i.e., Req.4) by considering problem space changes as part of its definition. 
%In order to account for solution space changes, we need to remove feature tuples that are affected by solution space changes between two commits (i.e., code changes from one commit to another) to prevent a false coverage estimate for those feature tuples.
%We introduce the preprocessing function $\pre$ to adjust the configurations contained in the sample window $\sampleWindowLHS$ before computing continuous t-wise coverage. 
%Our preprocessing function takes as input the sample window $\sampleWindowLHS$ and a set of changed features $\chf$. 
%The set of changed features can be identified using a change impact and dependency analysis on the solution space of the considered system. 
%Which change impact analysis approach is used to obtain the set of changed features is not relevant for our metric. 
%Therefore, we will not explore this topic further.
%The preprocessing function ($\preLHS$) removes all changed features contained in $\chfLHS$ from the configurations contained in the sample window $\sampleWindowLHS$. 
%This process may result in invalid configurations, which does not affect the calculation of continuous t-wise coverage because it considers the validity of feature tuples independent of configuration validity. 
%Applying $\preLHS$ before calculating continuous t-wise coverage ensures that all feature tuples considered in the calculation are not affected by changes in the solution (e.g., the feature code has not changed between commits). 
%Therefore, the combination of our metric definition and the introduced preprocessing function satisfies the second part of our robustness requirement (i.e., Requirement 4). 
%}

%\subsection{Conformance to the Requirements}
%\label{subsec:conformance}
%In the following, we discuss whether the defined metric conforms to the list of requirements described earlier.
%
%\paragraph{R1: Equivalence} The definition of continuous t-wise coverage is kept as close as possible to the metric for one-shot feature interaction coverage. We replace the single sample of one-shot sampling with a set of samples joined by the set union operation. Hence, by setting the size of $\commitWindowLHS$ to $\windowSizeLHS = 1$, we get the same results for continuous t-wise coverage as for one-shot coverage, which fulfills our first requirement.
%
%\paragraph{R2: Adaptability} Depending on the nature of development on a system, different commit-window sizes can be appropriate. Volatile systems for instance, with many small changes to the solution space in short time, will invalidate low numbers of sample configurations on each commit and will probably benefit from a large commit history. Reducing the number of samples tested for each commit, our metric can adapt to restrictive time and resource constraints and, more indirectly, the demands of the test suite being executed.
%
%Therefore, by adjusting both the size of the commit window $n$ and the number of considered samples $m$, our metric can adapt to the system at hand as well as the restrictions of the testing process, fulfilling our second requirement.
%
%\paragraph{R3: Tuple Uniqueness}
%As the function $I$ is defined using sets, computing the union of samples from the sample window yields itself a set of unique configurations, maintaining a correct number of covered interactions, even if they are covered by multiple sample configurations in different samples. Hence, we fulfill the third of our requirements by definition.
%
%\paragraph{R4: Robustness} As described in \autoref{subsec:confTest}, the formula $\interInSamLHS$ provides the set of all valid t-wise feature tuples for a feature model.
%Continuous t-wise coverage uses the same formula to get all valid t-wise feature tuples from a joined set of configurations (i.e., a sample).
%Hence, per definition all invalid feature tuples for the most-recent feature model, are excluded from the calculation of continuous t-wise coverage and our metric fulfill the fourth requirement.


==> 002_sections/problemstatement.tex <==
%% Introduction
Achieving t-wise feature interaction coverage over time by accumulating covered feature interactions for a number of previous commits (commit window) may reduce testing effort for a commit.
We show this potential by a thought experiment.

% Mind experiment
\paragraph{Thought Experiment}
Assume we have our running example from \autoref{fig:runningexamplenotfinal}, for which we want to ensure functional safety during the system's evolution.
Typically, the system developers commit three times a day, but the feature model is not changed.
The system needs to be tested with pair-wise feature interaction coverage for each commit.
Using the YASA sampling algorithm~\cite{KTS+:VaMoS20}, we calculate a pair-wise feature interaction sample containing seven configurations in less than 20 seconds.
However, we only have time to test three configurations per commit.
So, we cannot achieve full pairwise feature interaction coverage in one commit because we do not have the testing resources to fully test seven configurations.
%However, if we soften the requirement of achieving pair-wise coverage in every commit slightly to achieving coverage once per day, this becomes feasible.
%We can split up the seven configurations so that each is tested at least once after three commits.
However, if we soften the requirement of achieving pair-wise coverage in every commit slightly to achieving coverage once per day, this becomes feasible, by splitting the seven configurations so that each is tested at least once after three commits.

\begin{table}
	\caption{Configurations tested per commit of the evolution history of the running example.}
	\label{tab:exampSampleHistory}
	\begin{tabular}{c||c l}
		commit & \multicolumn{2}{c}{configuration}  \\ \hline
		& c1 & $\setOpen 0,1,\neg 2,3,\neg 4,\neg 5,\neg 6,7,\neg 8,\neg 9,\neg 10 \setClose$ \\
		commit 0 & c2 & $\setOpen 0,1,2,3,4,5,6,7,\neg 8,9,\neg 10 \setClose$ \\
		& c3 & $\setOpen 0,1,\neg 2,3,\neg 4,\neg 5,\neg 6,\neg 7,8,\neg 9,\neg 10 \setClose$ \\ \hline
		& c4 & $\setOpen 0,1,2,3,4,5,6,7,\neg 8,\neg 9,10 \setClose$ \\
		commit 1 & c5 & $\setOpen 0,1,2,3,4,\neg 5,\neg 6,\neg 7,8,9,10 \setClose$ \\
		& c6 & $\setOpen 0,1,2,3,\neg 4,\neg 5,6,\neg 7,8,\neg 9,\neg 10 \setClose$ \\ \hline
		%& c1 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\
		& c7 & $\setOpen 0,1,2,3,\neg 4,5,\neg 6,\neg 7,8,\neg 9,\neg 10 \setClose$ \\
		commit 2 & \textcolor{darkgray!90}{c1} & \textcolor{darkgray!90}{$\setOpen 0,1,\neg 2,3,\neg 4,\neg 5,\neg 6,7,\neg 8,\neg 9,\neg 10 \setClose$} \\
		& \textcolor{darkgray!90}{c2} & \textcolor{darkgray!90}{$\setOpen 0,1,2,3,4,5,6,7,\neg 8,9,\neg 10 \setClose$}
		%%& c3 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$
	\end{tabular}
\end{table}

% table description
\autoref{tab:exampSampleHistory} shows the mapping between commits and tested configurations.
The first column of the table shows the numbered commits from one to three, while the second column shows configurations with configuration names one to seven and the set of features contained by the configuration.
According to our testing requirements we can test three configurations per commit.
In commit 1 and 2, we test three configurations each.
So that, we need to test only one of those seven configurations in commit 3, which leaves testing resources for retesting configurations (e.g., c1 and c2).
\autoref{tab:exampSampleHistory} indicates that configurations c1 and c2 will be retested after the coverage threshold is reached. 
This is an example to illustrate how retesting of configurations can be done.	
In a real test scenario, the order of retesting configurations could be adjusted appropriately. 
\autoref{tab:exampSampleHistory} shows that it is possible to split a t-wise interaction sample over multiple commits to achieve t-wise feature interaction coverage after the third commit.
In practice, however, calculating a sample in advance and distributing the configurations of that sample across multiple commits is not useful due to changes in the problem space and solution space. 
Instead, samples of the required size are created for each commit individually. 
Calculating how much t-wise feature interaction coverage is achieved by samples of previous system versions is not possible with the currently established one-shot metric, at least not without addressing the following questions: 
1) For which feature model do we compute the t-wise feature interaction coverage? 
2) Which feature tuples are still valid for the chosen system version?
3) How can we make sure that feature tuples are not considered multiple times, thus inflating the t-wise interaction coverage?
%4) Which features cannot be considered covered due to changed solution space artifacts (i.e., source code changes)? (e.g., consideration of solution space changes)
With continuous t-wise coverage, we present a metric that addresses these questions and can that be applied to an evolution history of a configurable system.

%\paragraph{Requirements:}
However, simply accumulating t-wise feature interaction coverage over time is not yet sufficient.
In a real-world evolution scenario, there are significant challenges that must be addressed by a well defined metric.
For example, many of the current testing procedures focus on one-shot coverage, which should not be ignored by the new metric.
Therefore, we require \emph{equivalence (Req.1)} between one-shot coverage and continuous t-wise coverage to allow a seamless conversion of current procedures.
Depending on the nature and structure of the system and development process, real-world testing scenarios differ strongly wrt. quality demands and testing time. 
%Volatile systems for instance, with many small changes to the solution space in short time, will invalidate low numbers of sample configurations on each commit and will probably benefit from a large commit history.
For example, testing a volatile system with many small changes to the problem and solution space in a short period of time will invalidate previously covered feature tuples on each commit, and will likely not benefit from a large commit history. 
Instead, it will be more beneficial for these systems to test more new configurations, increasing the testing time per commit. 
On the other hand, for a stable system with few changes to the problem and solution space, covered feature tuples will remain valid for many commits in the commit history.
Therefore, testing these systems will benefit from considering longer commit histories and testing fewer configurations in each commit to spread the testing effort over time. 
%Continuous t-wise coverage must be applicable in any real-world testing scenarios, which demands customization options and high adaptability.
%We require \emph{adaptability (R2)} to testing requirements of different domains.
Therefore, we require that continuous t-wise coverage must be \emph{adaptable (Req.2)} wrt. the number of configurations tested in one commit, and the number of commits that are used to achieve t-wise feature interaction coverage over time.
During the evolution of configurable systems feature tuples may be covered by different configurations or become invalid because of changes to the problem or solution space of the system.
We require \emph{tuple uniqueness (Req.3)} and \emph{robustness (Req.4)} when calculating t-wise feature interaction coverage, so that duplicate and invalid feature tuples do not distort the result of continuous t-wise coverage.

==> 002_sections/problemstatement_draft.tex <==
%\section{Sample Based Testing for Evolving Systems is Difficult}
%In this section we elaborate why sample-base testing for evolving configurable systems is difficult. 
%We discuss the challenges of sample-based testing in continuous integration in \autoref{subsec::challenge}. 
%In \autoref{subsec::challengeMeasuring}, we elaborate the challenges of measuring t-wise feature interaction coverage during the evolution of a configurable system.
Today, many software intensive systems are not only configurable but also evolve frequently, adjusting to user and market changes. 
The frequent evolution is especially challenging when the software-intensive system is safety critical (e.g., subsystems of a car from automotive industry).
Those systems require an exhaustive testing process, which is not manageable for a frequent evolution of the system, not even by applying current sampling strategies.
In the following chapters we will discuss the challenges of frequently evolving systems to the verification of configurable systems and why the usage one-shot coverage is not enough for modern software development strategies. 
We start by discussing the process of evolving configurable systems frequently in \autoref{subsec:evo}. 
In \autoref{subsec:challenges} we elaborate on the challenge that arise when using one-shot coverage for sample-based testing of frequently evolving system.

%%-----------------------------------------------------------------
\subsection{Evolution of Configurable Systems}
\label{subsec:evo}
\todoTP{describe system version}
\todoTP{introduce term evolution step}
\todoTP{system history}
\todoTP{considered dimension / lookback}
\todoTP{introduce term Timestamp}
\todoTP{Describe CI Phases}
\todoTP{Describe why testing as subphase sampling in our case}
\todoTP{Evolution in Problem and Solution space}
\todoTP{sample historie}

%topic introduction
Modern day software intensive systems need to adapt to ever changing market and customer requirements.
This includes adapting the system's variability, the so called problem space (i.e., feature and their dependencies), as well as the system's functionality the so called solution space (i.e., the implementation artifacts mapped to the features)~\cite{KGS:SPLC18}.
We call the adaptation of problem or solution space the evolution of our configurable system. 
Changes to problem space are less frequent than changes to the implementation artifacts~\todoCite{Ref}. 

% ci cycle
Typically the evolution of a system includes four phases (develop, commit, integrate, and test)~\todoCite{CI}.
The process of evolving the system starts with a developer who changes the problem- or the solution space of the system (i.e, develop), and commits his changes to a repository (i.e., commit phase). 
Integrating the commit of the developer into the system creates a new system version (i.e., integrate).
For this paper we assume, that the integration of a commit happens automatically, so that a commit always creates a new system version.
The functionality of the system is then verified by testing (i.e., test), before the evolution process starts anew.

% commit history
Over time, a history of system versions (i.e., commit-history) is build by the developers of the system.
\begin{table}
	\caption{Documentation of system changes for the running example shown in \autoref{fig:runningexamplenotfinal}. An X indicates that a feature was changed in the respective commit.}
	\label{tab:exampEvoHistory} 
	\begin{tabular}{c||c|c|c}
		features & commit 1 & commit 2 & commit 3 \\ \hline
		\texttt{Car} & - & - & X \\
		\texttt{Carbody} & - & X & - \\
		\texttt{Radio} & - & - & X \\
		\texttt{Gearbox} & - & - & - \\
		\texttt{Ports} & - & X & - \\
		\texttt{Navigation} & - & X & - \\
		\texttt{Bluetooth} & X & - & - \\
		\texttt{Manual} & X & X & X \\
		\texttt{Automatic} & X & - & X \\
		\texttt{USB} & - & X & - \\
		\texttt{CD} & - & X & -
	\end{tabular}
\end{table}

\autoref{tab:exampEvoHistory} summarizes the changes of features during the evolution of our running example from \autoref{fig:runningexamplenotfinal}. 
In the first column of the table all features of the system are listed. 
The first row of the table the commits that form the evolution history of our running example.
We have four commits in this history. 
The cells of \autoref{tab:exampEvoHistory} indicate whether a feature was changed in the respective commit.
For instance, in the first commit the features \texttt{Bluetooth}, \texttt{Manual}, and \texttt{Automatic} were changed.
For running example we assume that only implementation artifacts of the system (i.e., the solution space) was changed.

\begin{table}
	\caption{Configurations tested per commit of the evolution history of the running example. \todoTP{Anpassen}}
	\label{tab:exampSampleHistory} 
	\begin{tabular}{c||c c}
		commit & & configuration \\ \hline
		& c1 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\
		commit 1 & c2 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\
		& c3 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\ \hline
		& c4 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\
		commit 2 & c5 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\
		& c6 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\ \hline
		%& c1 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ \\
		commit 3 & c7 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$ %\\
		%%& c3 & $\setOpen 0,1,2,3,4,5,6,\neg 7,8,9,10 \setClose$
	\end{tabular}
\end{table}
% sample based-testing
After a commit, the functional safety of the configurable system is typically verified by sample-based testing, regardless of whether the solution space, the problem space, or both were changed by the commit.
During sample-based testing, selected test cases are executed on selected system configurations (i.e., a test sample). 
The selection of test cases is out of scope for this paper, so we do not describe the selection process in detail. 

\todoTP{Kapitel noch mal Umdenken:
	\begin{itemize}
		\item Änderungen interessieren nicht für Metrik --> Commit Historie entfernen
		\item Festlegen auf nur solution space changes 
		\item Evolutionsprozess auch eher uninteressat für die Metrik. Wichtig es gibt evolution über commits, es sind meistens viele commits (Linux)
		\item Testen der commits erfolgt sample basiert, mit oft strengen Anforderungen an Qualität (t-wise coverage) und Testressourcen (nur bestimmte Anzahl an Commits testen, trotzdem hohe coverage)
		\item aktuelle Metrik für t-wise coverage nicht ausreichend, da nur one-shot coverage betrachtet (Nachweis an beispiel sample history)
		\item An unserem Running Example ist es möglich, coverage zu akkumulieren --> zeigen an beispiel
\end{itemize}}

% challenge in system testing
Modern configurable systems such as the Linux kernel evolve frequently with multiple commits per day. 
The Linux foundation measured over 75,000 commits per year in 2019 for the Linux kernel\footnote{\linuxAnualRep}. 
75,000 commits per year means that about 205 commits happen to the Linux kernel every day of the year.
Testing 205 commits per day leaves about seven minutes of testing time for each commit.
Securing the functional safety for a highly configurable system such as Linux with about \todoTP{aktuelle Anzahl} possible variants according to strict quality requirements (e.g., t-wise feature interaction coverage) in seven minutes is challenging.
Using a modern and efficient sampling algorithm such as YASA~\cite{KTS+:VaMoS20} the calculation of a pair-wise ($\twise = 2$) for an older version of Linux (i.e., Linux 2.6.6) takes about 34~minutes and results 500~configurations for testing.
Even by excluding the time to calculate a pair-wise sample, testing 500~configurations in about seven minutes is fairly infeasible because executing all test cases for a configuration cannot take longer than 0.84~seconds.
Following this reasoning, we deem sample-based testing according to high t-wise feature interaction values for each commit of frequently evolving configurable systems as infeasible.

% introducing the benefits of continuous coverage
However, do we need to achieve full t-wise feature interaction coverage for each commit of the? 
Or is it enough to achieve t-wise coverage once per day, once per week or even once per month, by accumulating the tested feature-interactions in the respective time span?
The current metric for t-wise feature interaction coverage does not allow the accumulation of feature interactions tested for past system versions.
Still, we think that the accumulation of covered t-wise feature interactions has potential to improve the quality of sample-based testing for frequently evolving configurable systems. 
We will show this potential in a small mind experiment using our running example. 

% Mind experiment
Assume we have our running example from \autoref{fig:runningexamplenotfinal}, for which we want to secure functional safety during the systems evolution.
Typically the system developers commit three times day (i.e., the system evolves three times a day), but the feature model is not changed.
We have strict testing requirements that the system needs to be tested with pair-wise feature interaction coverage for each commit.
Using the YASA sampling algorithm we calculate a pair-wise feature interaction sample, which contains seven configurations in less than 20 seconds. 
However, we only have time to test three configurations per commit. 
Using the current definition of t-wise feature interaction coverage, we cannot fulfill the test requirements, because we do not have the test resources (i.e., testing time) to test seven configurations.
However, if we soften the requirement of achieving t-wise coverage in every commit slightly to achieving the coverage once per day, the feasibility strongly increases.
In the setup of our mind experiment, we can split up the seven configurations required to achieve t-wise feature interaction coverage, so that after three days all of them are tested. 

% table describtion
\autoref{tab:exampSampleHistory} shows how the configurations are split to the commits. 
The first column of the table shows the numbered commits from one to three, while the second column shows configurations with configuration name one to seven and the set of features contain by the configuration. 
To visualize the set of contained features we use our shorthand notion. 
For commit one and two three configurations are displayed. 
For commit three one configuration is displayed, because we do not need more configurations to achieve pair-wise feature interaction coverage.
\autoref{tab:exampSampleHistory} shows that it is theoretically possible to split a t-wise interaction sample over multiple commits to achieve t-wise feature interaction coverage after the third commit. 

% Requirements for sample-based testing of safety critical systems
Our mind experiment is a strong simplification of a real-world evolution scenario.
We assume that configurations from a t-wise feature interaction sample can be used for all three commits, this is only possible when the systems variability is not affected by the commits. 
Otherwise invalid configurations and feature interactions may appear, that must be handled. 
We also work with fixed testing requirements that for our example.
In a real world setup the testing requirements may differ greatly from what we defined for our example with regard to the number of tested configurations per commit and the number of commits in which t-wise feature interaction coverage need to be achieved.
However, our mind experiment clearly shows the potential of accumulating t-wise feature interactions over time. 
We do not use a metric to calculate t-wise feature interaction coverage continuously, instead we split a sample from which we know that it achieves t-wise feature interaction coverage. 
In a real world setting this procedure is not applicable, and we need a well-defined metric to calculate continuous t-wise coverage.
The metric must conform to the following requirements:
\begin{itemize}
	\item Enable trade-off between number tested configurations per commit and number of system versions to reach 100\% t-wise coverage.
	\item Handle invalid feature interactions. 
	\item Handle duplicate configurations and feature interactions, between samples for different commits.
	\item Conform to the current metric for one-shot coverage, when calculating t-wise feature interaction coverage for one system version.
	\item \todoAll{More?}
\end{itemize}

%Highly configurable systems continuously evolve in the problem space (i.e., the system's features and dependencies) as well as in the solution space (i.e., the system's implementation artifacts)~\cite{KGS:SPLC18}. 
%An evolution of the problem space influences the variability of the system by applying feature model change operations (e.g., adding and removing features and feature dependencies)~\cite{TBK:ICSE09, BKL+:AUSE15}.
%The solution space evolves when developers add, remove, or update implementation artifacts of the system. 
%A modification of the solution space typically influences the concrete functionality of the system.
%Testing must be performed after each evolution step, regardless of whether the problem space or solution space is changed.
%Typically, testing the system after a problem space or solution space change requires re-sampling because configurations may have become invalid or new configurations may have been emerged based on the changes. 
%
%Configurable systems developed with continuous integration evolve in fast incremental update cycles \todo{Commits Linux per day}.
%After each cycle, the system's quality is assured by testing.
%In continuous integration an update cycle consists of four phases: 1) develop, 2) integrate, 3) commit, and 4) test~\cite{Sto+:AC09, DMG:07, Meyer:IEEESoftw.14}. 
%For sample-based testing in CI, a sample phase before testing is required, so that we define five phases for developing configurable systems with CI.

%%-----------------------------------------------------
\subsection{Challenges for Sample-Based Testing}
\label{subsec:challenges}
\todoTP{Finale Aussage: Hey, unsere aktuelle Metric ist nicht ausreichend, weil man selbst mit limitierter configurations Zahl, über die Zeit gute Coverage erreichen kann. Am Beispiel (Sample History zeigen)}
%Current sampling algorithms calculate samples that achieve t-wise feature interaction coverage in one-shot for each system version. 
%Those sampling algorithms often create large samples for which a complete test execution is not feasible in the limited testing time of continuous integration. 
%Therefore, sample-based testing with more than pair-wise feature interaction (t = 2) coverage is often not used.
%
%Imagine the following scenario for our running example.
%We need to use sample-based testing that achieves 4-wise feature interaction coverage to assure the functional safety of our system according to safety requirements in our department.
%However, testing time for the system is strictly limited, so that we can only test four configurations in one continuous integration cycle.
%Current state-of-the-art sampling algorithms such as YASA~\cite{KTS+:VaMoS20} can calculate a sample that achieves 4-wise feature interaction coverage for our running example, which consists of 20 configurations.
%
%In our example scenario, we can test 4 out of 20 configurations required to achieve 4-wise feature interaction coverage in one test cycle. 
%The system evolves during the development phase, and a new sample must be created for testing. 
%Again, only 4 out of 20 configurations can be tested, and this process repeats in each evolution cycle.
%
%A naive approach to addressing our example scenario's challenge is periodic testing of all configurations in a calculated sample. 
%For instance, we calculate a sample and test all of its configurations only after each fifth commit. 
%We achieve full 4-wise feature interaction coverage after each fifth commit. 
%However, we do not get any information about system faults for four commits, and the testing process in each fifth commit takes a long time. 
%Therefore, the naive approach of periodic testing is not practicable.
%
%Instead, we need an incremental sampling algorithm, that considers the limited testing time in continuous integration and that actively uses the fast update cycles of continuous integration to increase t-wise feature interaction coverage over time. 

%\subsection{Challenges of Measuring T-Wise Coverage during System Evolution}
%\label{subsec::challengeMeasuring}
%Measuring 
%\paragraph{Handling of invalid configurations}
%\paragraph{Keeping previous configurations}


==> 004_figures/carExample/backup/carExample.tex <==
\begin{forest}
	featureDiagram
	[Car [0],concrete[Carbody [1],concrete,mandatory][Radio [2],concrete,optional[Ports [4],concrete,optional[USB [9],concrete,or][CD [10],concrete]][Navigation [5],concrete,optional][Bluetooth [6],concrete,optional]][Gearbox [3],concrete,mandatory[Manual [7],concrete,alternative][Automatic [8],concrete]]]	
	\matrix [anchor=north west] at (current bounding box.north east) {
		\node [placeholder] {}; \\
	};
	\matrix [draw=drawColor,anchor=north west] at (current bounding box.north east) {
		\node [label=center:\underline{Legend:}] {}; \\
		\node [concrete,label=right:Feature] {}; \\
		\node [mandatory,label=right:Mandatory] {}; \\
		\node [optional,label=right:Optional] {}; \\
			\filldraw[drawColor] (0.1,0) - +(-0,-0.2) - +(0.2,-0.2)- +(0.1,0);
			\draw[drawColor] (0.1,0) -- +(-0.2, -0.4);
			\draw[drawColor] (0.1,0) -- +(0.2,-0.4);
			\fill[drawColor] (0,-0.2) arc (240:300:0.2);
		\node [or,label=right:Or Group] {}; \\			\draw[drawColor] (0.1,0) -- +(-0.2, -0.4);
			\draw[drawColor] (0.1,0) -- +(0.2,-0.4);
			\draw[drawColor] (0,-0.2) arc (240:300:0.2);
		\node [alternative,label=right:Alternative Group] {}; \\	};
\end{forest}

==> 004_figures/carExample/backup/head.tex <==
%---required packages & variable definitions------------------------------------
\usepackage{forest}
\usepackage{xcolor}
\usetikzlibrary{angles}
\definecolor{drawColor}{RGB}{128 128 128}
\newcommand{\circleSize}{0.25em}
\newcommand{\angleSize}{0.8em}
%-------------------------------------------------------------------------------
%---Define the style of the tree------------------------------------------------
\forestset{
	/tikz/mandatory/.style={
		circle,fill=drawColor,
		draw=drawColor,
		inner sep=\circleSize
	},
	/tikz/optional/.style={
		circle,
		fill=white,
		draw=drawColor,
		inner sep=\circleSize
	},
	featureDiagram/.style={
		for tree={
			text depth = 0,
			parent anchor = south,
			child anchor = north,
			draw = drawColor,
			edge = {draw=drawColor},
		}
	},
	/tikz/abstract/.style={
		fill = blue!85!cyan!5,
		draw = drawColor
	},
	/tikz/concrete/.style={
		fill = blue!85!cyan!20,
		draw = drawColor
	},
	mandatory/.style={
		edge label={node [mandatory] {} }
	},
	optional/.style={
		edge label={node [optional] {} }
	},
	or/.style={
		tikz+={
			\path (.parent) coordinate (A) -- (!u.children) coordinate (B) -- (!ul.parent) coordinate (C) pic[fill=drawColor, angle radius=\angleSize]{angle};
		}	
	},
	/tikz/or/.style={
	},
	alternative/.style={
		tikz+={
			\path (.parent) coordinate (A) -- (!u.children) coordinate (B) -- (!ul.parent) coordinate (C) pic[draw=drawColor, angle radius=\angleSize]{angle};
		}	
	},
	/tikz/alternative/.style={
	},
	/tikz/placeholder/.style={
	},
	collapsed/.style={
		rounded corners,
		no edge,
		for tree={
			fill opacity=0,
			draw opacity=0,
			l = 0em,
		}
	},
	/tikz/hiddenNodes/.style={
		midway,
		rounded corners,
		draw=drawColor,
		fill=white,
		minimum size = 1.2em,
		minimum width = 0.8em,
		scale=0.9
	},
}
%-------------------------------------------------------------------------------


==> 004_figures/carExample/carExample.tex <==
\begin{forest}
	featureDiagram
	[Car, concrete[Carbody, concrete, mandatory][Radio, concrete, optional[Ports, concrete, optional [USB ,concrete, or][CD,concrete]][Navigation, concrete, optional][Bluetooth, concrete, optional]][Gearbox, concrete, mandatory[Manual ,concrete, alternative][Automatic, concrete]]]	
	\matrix [anchor=north west] at (current bounding box.north east) {
		\node [placeholder] {}; \\
	};
	\matrix [draw=drawColor,anchor=north west] at (current bounding box.north east) {
		\node [label=center:\underline{Legend:}] {}; \\
		\node [concrete,label=right:Feature] {}; \\
		\node [mandatory,label=right:Mandatory] {}; \\
		\node [optional,label=right:Optional] {}; \\
			\filldraw[drawColor] (0.1,0) - +(-0,-0.2) - +(0.2,-0.2)- +(0.1,0);
			\draw[drawColor] (0.1,0) -- +(-0.2, -0.4);
			\draw[drawColor] (0.1,0) -- +(0.2,-0.4);
			\fill[drawColor] (0,-0.2) arc (240:300:0.2);
		\node [or,label=right:Or Group] {}; \\			\draw[drawColor] (0.1,0) -- +(-0.2, -0.4);
			\draw[drawColor] (0.1,0) -- +(0.2,-0.4);
			\draw[drawColor] (0,-0.2) arc (240:300:0.2);
		\node [alternative,label=right:Alternative Group] {}; \\	};
\end{forest}

==> 004_figures/fig_coverage_t2_accu.tex <==
\begin{figure}[h!]
    \centering
    %\includegraphics[width=0.80\linewidth]{../004_figures/plots/t2_coverage/coverage_t2_short.pdf}
    \includegraphics[width=0.7\textwidth]{./004_figures/plots/t2_coverage/coverage_t2.pdf}
    \caption{Results of measuring pair-wise ($\twise = 2$) coverage.
    %feature interaction coverage of our experiment execution. 
    %Each box represents results measured for the respective experiment (Label on the X-Axis). The boxes aggregate the results measured for all subject systems.
    }
    \label{fig:T2_coverage}
\end{figure}

==> 004_figures/fig_coverage_t3_accu.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{../004_figures/plots/t3_coverage/coverage_t3.pdf}
    %\includegraphics[width=0.80\linewidth]{../004_figures/plots/t3_coverage/coverage_t3_short.pdf}
    \caption{Results of measuring three-wise ($\twise = 3$) coverage.
    %feature interaction coverage of our experiment execution. Each box represents results measured for the respective experiment (Label on the X-Axis). The boxes aggregate the results measured for all subject systems.
    }
    \label{fig:T3_coverage}
\end{figure}

==> 004_figures/fig_size_accu.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{../004_figures/plots/size/sample_size.pdf}
    %\includegraphics[width=0.80\linewidth]{../004_figures/plots/size/sample_size_short.pdf}
    \caption{Results of measuring the sample size. 
    %of the samples resulting from executing our experiments. Each box represents results measured for the respective experiment configuration (Label on the X-Axis). The boxes aggregate the results measured for all subject systems.
    }
    \label{fig:size}
\end{figure}

==> 004_figures/fig_time_accu.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{../004_figures/plots/time/total_time.pdf}
    %\includegraphics[width=0.80\linewidth]{../004_figures/plots/time/total_time_short.pdf}
    \caption{Results of measuring sampling time.
    %for our experiment configurations. %Each box represents results measured for the respective experiment configuration (Label on the X-Axis). The boxes aggregate the results measured for all subject systems.
    }
    \label{fig:time}
\end{figure}

==> 004_tables/attributes_example.tex <==
\begin{table}
	\centering
	\caption{Attribute table that shows randomly assigned attributes for each feature of our running example.}
	\begin{tabular}[t]{llr} 
		\toprule
		literal 	& feature name 			& attribute value 
		\\ \toprule
		0 			& Car 					& 2 \\
		1 			& Carbody 				& 3	\\
		2 			& Radio 				& 4 \\
		3 			& Gearbox 				& 2 \\
		4 			& Ports 				& 1 \\
		5 			& Navigation			& 4 \\
		6 			& Bluetooth 			& 2 \\
		7 			& Manual 				& 3 \\
		8 			& Automatic 			& 4 \\
		9 			& USB 					& 3 \\
		10 			& CD 					& 4 \\ 
		\bottomrule	
	\end{tabular}
	\label{tab:attributeTable}
\end{table}
